Digital Contact Tracing Service: An improved decentralized design for privacy and effectiveness

We propose a decentralized digital contact tracing service that preserves the users' privacy by design while complying to the highest security standards. Our approach is based on Bluetooth and measures actual encounters of people, the contact time period, and estimates the proximity of the contact. We trace the users' contacts and the possible spread of infectious diseases while preventing location tracking of users, protecting their data and identity. We verify and improve the impact of tracking based on epidemiological models. We compare a centralized and decentralized approach on a legal perspective and find a decentralized approach preferable considering proportionality and data minimization.

==> openQuestions.tex <==
\section{Open Questions \label{sec:questions}}
\subsection{Is there a better protocol, which enables second order tracing?}
\subsection{How to avoid rebroadcasting of already uploaded IDs?}
\subsection{For private set intersections: how computationally expensive is it? What are good values for $k, m$ (and what is a proper hash) of the Bloom filter in order to have a low false positive rate?}

